Reliable Transiently-Powered Communication

Frequent power failures can introduce significant packet losses during communication among energy harvesting batteryless wireless sensors. Nodes should be aware of the energy level of their neighbors to guarantee the success of communication and avoid wasting energy. This paper presents TRAP (TRAnsiently-powered Protocol) that allows nodes to communicate only if the energy availability on both sides of the communication channel is sufficient before packet transmission. TRAP relies on a novel modulator circuit, which operates without microcontroller intervention and transmits the energy status almost for free over the radiofrequency backscatter channel. Our experimental results showed that TRAP avoids failed transmissions introduced by the power failures and ensures reliable intermittent communication among batteryless sensors.

==> 7-biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Alessandro_Torrisi.jpg}}]{Alessandro Torrisi} received his M. S. degree in Electronic Engineering at the University of Padova, Italy, in 2019 (cum laude). During the last M.S. year, he was an Erasmus student at the Technische Universität of Vienna, Austria, where he developed his M.S. thesis project. Currently, he is pursuing a Ph.D. at the Department of Industrial Engineering at the University of Trento, Italy. His research activities focus on the design of electronics, hardware and firmware, for the Internet of Things, especially, looking at the low power and constrained environment. At the moment, he is working on a zero-power communication mechanism for batteryless devices exploiting the backscatter technologies. He is a IEEE student member.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Kasim_Sinan_Yildirim.jpeg}}]{Kas{\i}m Sinan Y{\i}ld{\i}r{\i}m} received the MSc and PhD degrees in computer engineering from Ege University, Turkey, in 2006 and 2012, respectively. Currently, he is an assistant professor with the Department of Information Engineering and Computer Science, University of Trento, Italy. His research interests include embedded systems, intermittent computing, wireless networks, and distributed algorithms. He is a member of the IEEE.

 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{authors/Davide_Brunelli.png}}]{Davide Brunelli}
received his M.S. (cum laude) and Ph.D. degrees in electrical engineering from the University of Bologna, Italy, in 2002 and 2007, respectively.
He is currently an associate professor at the University of Trento, Italy. 
His research interests include IoT and distributed lightweight unmanned aerial vehicles UAV, the development of new techniques of energy scavenging for low-power embedded systems and energy-neutral wearable devices. 
He was leading industrial cooperation activities with Telecom Italia, ENI, and STMicroelectronics.
He has published more than 200 papers in international journals or proceedings of international conferences. He is an ACM member and a senior IEEE member.
\end{IEEEbiography}


